Position Reconstruction in LUX

The $(x, y)$ position reconstruction method used in the analysis of the complete exposure of the Large Underground Xenon (LUX) experiment is presented. The algorithm is based on a statistical test that makes use of an iterative method to recover the photomultiplier tube (PMT) light response directly from the calibration data. The light response functions make use of a two dimensional functional form to account for the photons reflected on the inner walls of the detector. To increase the resolution for small pulses, a photon counting technique was employed to describe the response of the PMTs. The reconstruction was assessed with calibration data including ${}^{\mathrm{83m}}$Kr (releasing a total energy of 41.5 keV) and ${}^{3}$H ($\beta^-$ with Q = 18.6 keV) decays, and a deuterium-deuterium (D-D) neutron beam (2.45 MeV). In the horizontal plane, the reconstruction has achieved an $(x, y)$ position uncertainty of $\sigma$= 0.82 cm for events of only 200 electroluminescence photons and $\sigma$ = 0.17 cm for 4,000 electroluminescence photons. Such signals are associated with electron recoils of energies $\sim$0.25 keV and $\sim$10 keV, respectively. The reconstructed position of the smallest events with a single electron emitted from the liquid surface has a horizontal $(x, y)$ uncertainty of 2.13 cm.

==> packages/hepparticles.tex <==
%% hepparticles --- flexible elementary particle symbols
%% Author: Andy Buckley <andy@insectnation.org>
%%
%% This material is subject to the LaTeX Project Public License.
%% See http://www.ctan.org/tex-archive/help/Catalogue/licenses.lppl.html
%% for the details of that license.
%%
%%
%% The macros provided are:
%%
%% For generic particle names e.g. all positively charged leptons:
%%   \HepGenParticle{main}{subscript}{superscript}
%%   \HepGenAntiParticle{main}{subscript}{superscript}
%%
%% For concrete particle names:
%%   \HepParticle{main}{subscript}{superscript}
%%   \HepAntiParticle{main}{subscript}{superscript}
%%
%% For supersymmetric "sparticles":
%%   \HepSusyParticle{main}{subscript}{superscript}
%%   \HepGenSusyParticle{main}{subscript}{superscript}
%%   \HepSusyAntiParticle{main}{subscript}{superscript}
%%   \HepGenSusyAntiParticle{main}{subscript}{superscript}
%%
%% For resonance specifiers (just the extra terms):
%%   \HepResonanceMassTerm{mainTermInParenths}{subscript}{superscript}
%%   \HepResonanceSpecTerm{mainSpecTerm}{subscript}{superscript}
%%
%% For the total particle name and resonance specifications: the
%% ``formal'' definitions include the spectroscopic term and the
%% ``full'' versions pf each require the main particle name to be
%% explicitly specified rather than just pass a \HepParticle as the first arg:
%%   \HepParticleResonance{name}{mass}{massSub}{massSup}
%%   \HepParticleResonanceFormal{name}{mass}{massSub}\
%%                              {massSup}{spec}{specSub}{specSup}
%%   \HepParticleResonanceFull{name}{sub}{sup}{mass}{massSub}{massSup}
%%   \HepParticleResonanceFormalFull{name}{sub}{sup}\
%%                                  {mass}{massSub}{massSup}\
%%                                  {spec}{specSub}{specSup}
%%
%% And finally, for containing processes describing the evolution
%% of these particles:
%%   \HepProcess{iParticles \to fParticles}
%% where \to is re-defined to have a bit of extra space.
%%
%% There are probably some missing cases but they can be handled
%% as explicit exceptions. You might also be interested in the
%% ``hepnames'' package, which updates the "pennames" set of
%% typeset concrete particle names to use this more flexible scheme.

%% TODO:
%%
%%  * Make the bold math only occur within particle macros
%%
%%  * Distinction between italic main symbol and italic main+scripts
%%
%%  * Optionally include Greek letters (lower and upper) in upright/italic
%%    forcing (and sans/bold context sensitivity)
%%
%%  * Use maybemath again? (A new version, using NFSS properly)

%% Admin
\def\fileversion{2.1}
\def\filedate{2015/10/20}
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{./hepparticles}[\filedate\space HEP particle typesetting (v\fileversion)]

% \RequirePackage{xspace}
% \RequirePackage{etoolbox}

%% Package options
\def\@italicNames{}%

%% Use italic particle symbols
\DeclareOption{italic}{%
  \def\@italicNames{yes}%
}
% %% Force particle symbols to behave as for italic math mode
% % TODO: clarify... means that text super/sub scripts are italic not rm?
% \DeclareOption{itforce}{%
%   \def\@italicNames{yes}%
%   \def\@forceItalic{yes}%
% }
% %% Force upright particle names (default)
% \DeclareOption{notitalic}{%
%   \def\@italicNames{}%
%   \def\@forceItalic{}%
% }
% %% Allow particle names to be sans-serif in context (no italics, even for generic particles)
% \DeclareOption{maybess}{%
%   \def\@maybeSansSerif{yes}%
% }
% \DeclareOption{noss}{%
%   \def\@maybeSansSerif{}%
% }

% TODO: Add options to force upright Greek lower-case / italic Greek upper-case?

\ProcessOptions

%% Force all sub/superscripts to the same height
\RequirePackage{subdepth}
\RequirePackage{amsmath}

%% Automatically bolden math mode symbols in a bold text context
% TODO: only apply to particles? Redefine \bfseries inside hepparticles macros and restore at end? Or is there a simpler scoping?
\g@addto@macro\bfseries{\boldmath}

\DeclareMathAlphabet{\mathup}{OT1}{\familydefault}{m}{n}
\SetMathAlphabet{\mathup}{bold}{\encodingdefault}{\familydefault}{bx}{n}

\DeclareMathAlphabet{\mathsfup}{OT1}{\sfdefault}{m}{n}
\SetMathAlphabet{\mathsfup}{bold}{\encodingdefault}{\sfdefault}{bx}{n}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{sl}

% \DeclareMathAlphabet{\mathbfsfit}{\encodingdefault}{\sfdefault}{bx}{sl} % why doesn't this work (no italic)?
% \DeclareMathAlphabet{\mathbfsf}  {\encodingdefault}{\sfdefault}{bx}{sl}

% TODO: Use fixmath to force italic/upright upper/lower Greek characters -- only in particles


%% -----------------------------------------------------------------------
%% Styling commands
%% -----------------------------------------------------------------------

%% Generic particle style (normal style with optional forced italics)
\DeclareRobustCommand{\@HepGenStyle}[1]{%
  \ensuremath{%
    \edef\@itcode{\itdefault}%
    \edef\@slcode{\sldefault}%
    \edef\@sfcode{\sfdefault}%
    \edef\@upcode{\updefault}%
    \edef\@bfcode{\bfdefault}%
    %
    \ifx\f@family\@sfcode%
      % \ifx\f@shape\@itcode%
      %   \ifx\f@series\@bfcode\bm{\mathsfit{#1}}\else\mathsfit{#1}\fi%
      % \fi%
      % \ifx\f@shape\@slcode%
      %   \mathsfit{#1}%
      % \fi%
      % \ifx\f@shape\@upcode%
      %   \mathsfup{#1}%
      % \fi%
%
      % \ifx\f@series\@bfcode\mathbfsf{#1}\else\mathsfit{#1}\fi%
%
      \mathsfit{#1}%
    \else%
      % \ifx\f@shape\@itcode%
      %   \mathit{#1}%
      % \fi%
      % \ifx\f@shape\@slcode%
      %   \mathit{#1}%
      % \fi%
      % \ifx\f@shape\@upcode%
      %   {#1}%
      % \fi%
%
      % \ifx\f@series\@bfcode\bm{\mathit{#1}}\else\mathit{#1}\fi%
%
      \mathit{#1}%
    \fi%
  }%
}


%% Concrete particle style (normal style with upright and forced italic handling)
\DeclareRobustCommand{\@HepConStyle}[1]{%
  \ensuremath{%
    \edef\@itcode{\itdefault}%
    \edef\@slcode{\sldefault}%
    \edef\@sfcode{\sfdefault}%
    \edef\@upcode{\updefault}%
    %
    \ifx\f@family\@sfcode%
      \ifx\f@shape\@itcode%
        \mathsfit{#1}%
      \fi%
      \ifx\f@shape\@slcode%
        \mathsfit{#1}%
      \fi%
      \ifx\f@shape\@upcode%
        \mathsfup{#1}% <--- difference from gen style
      \fi%
    \else%
      \ifx\f@shape\@itcode%
        \mathit{#1}%
      \fi%
      \ifx\f@shape\@slcode%
        \mathit{#1}%
      \fi%
      \ifx\f@shape\@upcode%
        \mathup{#1}% <--- difference from gen style
      \fi%
    \fi%
  }%
}


%% -----------------------------------------------------------------------
%% Conditional horizontal shifting and kerning for sub/superscripts
%% -----------------------------------------------------------------------

\DeclareRobustCommand{\@itmkern}[1]{%
  \ensuremath{%
    \edef\@itcode{\itdefault}%
    \edef\@slcode{\sldefault}%
    \edef\@sfcode{\sfdefault}%
    %
    \ifx\f@shape\@itcode%
      \mkern#1%
    \fi%
    \ifx\f@shape\@slcode%
      \mkern#1%
    \fi%
    \ifx\f@family\@sfcode%
      \mkern#1%
    \fi%
  }%
}

\DeclareRobustCommand{\@itsfshift}[2]{%
  \ensuremath{%
    \edef\@itcode{\itdefault}%
    \edef\@slcode{\sldefault}%
    \edef\@sfcode{\sfdefault}%
    \edef\@upcode{\updefault}%
    \edef\@bfcode{\bfdefault}%
    %
    \ifx\f@family\@sfcode%
      \ifx\f@shape\@itcode%
        \mspace{#2}
      \fi%
      \ifx\f@shape\@slcode%
        \mspace{#2}%
      \fi%
      \ifx\f@shape\@upcode%
        \relax%
      \fi%
    \else%
      \ifx\f@shape\@itcode%
        \mspace{#1}
      \fi%
      \ifx\f@shape\@slcode%
        \mspace{#1}
      \fi%
      \ifx\f@shape\@upcode%
        \relax%
      \fi%
    \fi%
  }%
}

\DeclareRobustCommand{\@sfshift}[2]{%
  \ensuremath{%
    \edef\@sfcode{\sfdefault}%
    %
    \ifx\f@family\@sfcode%
      \mspace{#2}
    \else%
      \mspace{#1}
    \fi%
  }%
}


%% -----------------------------------------------------------------------
%% Public commands for particle typesetting
%% -----------------------------------------------------------------------

%% For generic particles like "lepton", "quark" etc (no upright font)
\def\@shiftlen@norm@gen@rmsub{-3mu}
\def\@shiftlen@norm@gen@sfsub{-2mu}
\def\@shiftlen@norm@gen@rmsup{-1mu}
\def\@shiftlen@norm@gen@sfsup{0mu}
%
\DeclareRobustCommand{\HepGenParticle}[3]{%
  \@HepGenStyle{{#1}{}%
    _{\@sfshift{\@shiftlen@norm@gen@rmsub}{\@shiftlen@norm@gen@sfsub}\scriptstyle{#2}}%
    ^{\@sfshift{\@shiftlen@norm@gen@rmsup}{\@shiftlen@norm@gen@sfsup}\scriptstyle{#3}}}%
}
%% For generic antiparticles
\def\@shiftlen@anti@gen@bar{4mu}
\def\@shiftlen@anti@gen@rmsub{-2mu}
\def\@shiftlen@anti@gen@sfsub{-1mu}
\def\@shiftlen@anti@gen@rmsup{0mu}
\def\@shiftlen@anti@gen@sfsup{1mu}
%
\DeclareRobustCommand{\HepGenAntiParticle}[3]{%
  \@HepGenStyle{{\mkern\@shiftlen@anti@gen@bar\overline{\mkern-\@shiftlen@anti@gen@bar{#1}}}{}%
    _{\@sfshift{\@shiftlen@anti@gen@rmsub}{\@shiftlen@anti@gen@sfsub}\scriptstyle{#2}}%
    ^{\@sfshift{\@shiftlen@anti@gen@rmsup}{\@shiftlen@anti@gen@sfsup}\scriptstyle{#3}}}%
}

%% For generic SUSY particles e.g. slepton, squark
% cm/lmodern
\def\@shiftlen@susy@gen@til{2mu}
\def\@shiftlen@susy@gen@rmsub{-2.5mu}
\def\@shiftlen@susy@gen@sfsub{-2mu}
\def\@shiftlen@susy@gen@rmsup{-0.5mu}
\def\@shiftlen@susy@gen@sfsup{0mu}
% mathpazo
% \def\@shiftlen@susy@gen@til{2mu}
% \def\@shiftlen@susy@gen@rmsub{-1.5mu}
% \def\@shiftlen@susy@gen@sfsub{-2mu}
% \def\@shiftlen@susy@gen@rmsup{0.5mu}
% \def\@shiftlen@susy@gen@sfsup{0mu}
%
\DeclareRobustCommand{\HepGenSusyParticle}[3]{%
  \@HepGenStyle{{\mkern\@shiftlen@susy@gen@til\widetilde{\mkern-\@shiftlen@susy@gen@til{#1}}}{}%
    _{\@sfshift{\@shiftlen@susy@gen@rmsub}{\@shiftlen@susy@gen@sfsub}\scriptstyle{#2}}%
    ^{\@sfshift{\@shiftlen@susy@gen@rmsup}{\@shiftlen@susy@gen@sfsup}\scriptstyle{#3}}}%
}

%% For generic SUSY anti-particles e.g. slepton, squark
% cm/lmodern
\def\@shiftlen@antisusy@gen@bar{3.5mu}
\def\@shiftlen@antisusy@gen@til{2mu}
\def\@shiftlen@antisusy@gen@rmsub{-4mu}
\def\@shiftlen@antisusy@gen@sfsub{-3mu}
\def\@shiftlen@antisusy@gen@rmsup{-2mu}
\def\@shiftlen@antisusy@gen@sfsup{0mu}
% mathpazo
% \def\@shiftlen@antisusy@gen@bar{3.5mu}
% \def\@shiftlen@antisusy@gen@til{2mu}
% \def\@shiftlen@antisusy@gen@rmsub{-2mu}
% \def\@shiftlen@antisusy@gen@sfsub{-3mu}
% \def\@shiftlen@antisusy@gen@rmsup{0.7mu}
% \def\@shiftlen@antisusy@gen@sfsup{0mu}
%
\DeclareRobustCommand{\HepGenSusyAntiParticle}[3]{%
  %\@HepGenStyle{{\mkern3.5mu\overline{\mkern-1.5mu\widetilde{\mkern-2mu{#1}}}}{}%
  \@HepGenStyle{{\mkern\@shiftlen@antisusy@gen@bar\overline{\mkern-\@shiftlen@antisusy@gen@bar\mkern\@shiftlen@antisusy@gen@til\widetilde{\mkern-\@shiftlen@antisusy@gen@til{#1}}}}{}%
    _{\@sfshift{\@shiftlen@antisusy@gen@rmsub}{\@shiftlen@antisusy@gen@sfsub}\scriptstyle{#2}}%
    ^{\@sfshift{\@shiftlen@antisusy@gen@rmsup}{\@shiftlen@antisusy@gen@sfsup}\scriptstyle{#3}}}%
}



%% For concrete HEP particle names like "B", "J/psi" etc
% cm/lmodern
\def\@shiftlen@norm@con@rmsub{-2mu}
\def\@shiftlen@norm@con@sfsub{-1.5mu}
\def\@shiftlen@norm@con@rmsup{0mu}
\def\@shiftlen@norm@con@sfsup{0mu}
% mathpazo
% \def\@shiftlen@norm@con@rmsub{-3mu}
% \def\@shiftlen@norm@con@sfsub{-2mu}
% \def\@shiftlen@norm@con@rmsup{-1mu}
% \def\@shiftlen@norm@con@sfsup{0mu}
%
\DeclareRobustCommand{\HepParticle}[3]{%
  \ifx\@italicNames\@empty%
    \@HepConStyle{{{#1}}{}%
      _{\@itsfshift{\@shiftlen@norm@con@rmsub}{\@shiftlen@norm@con@sfsub}\scriptstyle{#2}}%
      ^{\@itsfshift{\@shiftlen@norm@con@rmsup}{\@shiftlen@norm@con@sfsup}\scriptstyle{#3}}}%
  \else%
    \HepGenParticle{#1}{#2}{#3}%
  \fi%
}
\DeclareRobustCommand{\HepIsotope}[3]{%
  \@HepConStyle{%
  _{\scriptstyle{#2}}%
  ^{\scriptstyle{#3}}%
   {#1}}}
%
\DeclareRobustCommand{\HepChemical}[3]{%
    \@HepConStyle{{{#1}}{}%
      _{\@itsfshift{\@shiftlen@norm@con@rmsub}{\@shiftlen@norm@con@sfsub}\scriptstyle{#2}}%
      ^{\@itsfshift{\@shiftlen@norm@con@rmsup}{\@shiftlen@norm@con@sfsup}\scriptstyle{#3}}}%
}
\DeclareRobustCommand{\HepGenParticle}[3]{%
  \@HepGenStyle{{#1}{}%
    _{\@sfshift{\@shiftlen@norm@gen@rmsub}{\@shiftlen@norm@gen@sfsub}\scriptstyle{#2}}%
    ^{\@sfshift{\@shiftlen@norm@gen@rmsup}{\@shiftlen@norm@gen@sfsup}\scriptstyle{#3}}}%
}

%% For concrete antiparticles
\def\@shiftlen@anti@con@bar{3.5mu}
\def\@shiftlen@anti@con@rmsub{-3mu}
\def\@shiftlen@anti@con@sfsub{-3mu}
\def\@shiftlen@anti@con@rmsup{1mu}
\def\@shiftlen@anti@con@sfsup{1mu}
%
\DeclareRobustCommand{\HepAntiParticle}[3]{%
  \ifx\@italicNames\@empty%
    \@HepConStyle{{\@itmkern{\@shiftlen@anti@con@bar}\overline{\@itmkern{-\@shiftlen@anti@con@bar}{#1}}}{}%
      _{\@itsfshift{\@shiftlen@anti@con@rmsub}{\@shiftlen@anti@con@sfsub}\scriptstyle{#2}}%
      ^{\@itsfshift{\@shiftlen@anti@con@rmsup}{\@shiftlen@anti@con@sfsup}\scriptstyle{#3}}}%
  \else%
    \HepGenAntiParticle{#1}{#2}{#3}%
  \fi%
}

%% For SUSY particles
% cm/lmodern
\def\@shiftlen@susy@con@til{2mu}
\def\@shiftlen@susy@con@rmsub{-3mu}
\def\@shiftlen@susy@con@sfsub{-3mu}
\def\@shiftlen@susy@con@rmsup{0mu}
\def\@shiftlen@susy@con@sfsup{0mu}
% mathpazo
% \def\@shiftlen@susy@con@til{2mu}
% \def\@shiftlen@susy@con@rmsub{-1mu}
% \def\@shiftlen@susy@con@sfsub{-2mu}
% \def\@shiftlen@susy@con@rmsup{1mu}
% \def\@shiftlen@susy@con@sfsup{0.5mu}
%
\DeclareRobustCommand{\HepSusyParticle}[3]{%
  \ifx\@italicNames\@empty%
    \@HepConStyle{{\@itmkern{\@shiftlen@susy@con@til}\widetilde{\@itmkern{-\@shiftlen@susy@con@til}{#1}}}{}%
      _{\@itsfshift{\@shiftlen@susy@con@rmsub}{\@shiftlen@susy@con@sfsub}\scriptstyle{#2}}%
      ^{\@itsfshift{\@shiftlen@susy@con@rmsup}{\@shiftlen@susy@con@sfsup}\scriptstyle{#3}}}%
  \else%
    \HepGenSusyParticle{#1}{#2}{#3}%
  \fi%
}

%% For SUSY anti-particles
% cm/lmodern
\def\@shiftlen@antisusy@con@bar{3.5mu}
\def\@shiftlen@antisusy@con@til{2mu}
\def\@shiftlen@antisusy@con@rmsub{-2.5mu}
\def\@shiftlen@antisusy@con@sfsub{-2mu}
\def\@shiftlen@antisusy@con@rmsup{0mu}
\def\@shiftlen@antisusy@con@sfsup{0mu}
% mathpazo
% \def\@shiftlen@antisusy@con@bar{3.5mu}
% \def\@shiftlen@antisusy@con@til{2mu}
% \def\@shiftlen@antisusy@con@rmsub{-2.5mu}
% \def\@shiftlen@antisusy@con@sfsub{-3mu}
% \def\@shiftlen@antisusy@con@rmsup{0mu}
% \def\@shiftlen@antisusy@con@sfsup{0mu}
%
\DeclareRobustCommand{\HepSusyAntiParticle}[3]{%
  \ifx\@italicNames\@empty%
    \@HepConStyle{{\@itmkern{\@shiftlen@antisusy@con@bar}\overline{\@itmkern{-\@shiftlen@antisusy@con@bar}%
                   \@itmkern{\@shiftlen@antisusy@con@til}\widetilde{\@itmkern{-\@shiftlen@antisusy@con@til}{#1}}}}{}%
      _{\@itsfshift{\@shiftlen@antisusy@con@rmsub}{\@shiftlen@antisusy@con@sfsub}\scriptstyle{#2}}%
      ^{\@itsfshift{\@shiftlen@antisusy@con@rmsup}{\@shiftlen@antisusy@con@sfsup}\scriptstyle{#3}}}%
  \else%
    \HepGenSusyAntiParticle{#1}{#2}{#3}%
  \fi%
}


%% Resonances and other such structures. These are actually pretty
%% complicated since the most general structure has a main particle
%% term, a mass term and a spectroscopic term: in total 9 possible arguments
%% if we let each main term have optional following sub- and super-scripts!
%% The mass and spectroscopic terms seem to be mixed up quite often... *sigh*
%%
%% Apologies for the interface changing yet again as I learn how general
%% these terms can be! Hopefully stable now (touch wood)...

%% For resonance mass specifications like the bracket in "J/psi(1S)"
\DeclareRobustCommand{\HepResonanceMassTerm}[3]{%
  \ifx\@italicNames\@empty%
    \@HepConStyle{{\left({#1}\right)}{}_{#2}^{\scriptstyle{#3}}}%
  \else%
    \@HepGenStyle{{\left({#1}\right)}{}_{#2}^{\scriptstyle{#3}}}%
  \fi%
}

%% For resonance spectroscopic specifications like the P_11 in "N(1440)P_11"
\DeclareRobustCommand{\HepResonanceSpecTerm}[3]{%
  \ifx\@italicNames\@empty%
    \@HepConStyle{{#1}{}_{#2}^{#3}}%
  \else%
    \@HepGenStyle{{#1}{}_{#2}^{#3}}%
  \fi%
}

%% For resonances like "J/psi(1S)" (first arg is a whole \HepParticle)
\DeclareRobustCommand{\HepParticleResonance}[4]{%
  \ensuremath{%
    {#1}{\HepResonanceMassTerm{#2}{#3}{#4}}%
  }%
}

%% For resonances like "N(1440)P_11" (first arg is a whole \HepParticle)
\DeclareRobustCommand{\HepParticleResonanceFormal}[7]{%
  \ensuremath{%
    {\HepParticleResonance{#1}{#2}{#3}{#4}}\,{\HepResonanceSpecTerm{#5}{#6}{#7}}%
  }%
}

%% For resonances like "J/psi(1S)" (all arguments ``spelled out'')
\DeclareRobustCommand{\HepParticleResonanceFull}[6]{%
  \HepParticleResonance{\HepParticle{#1}{#2}{#3}}{#4}{#5}{#6}%
}

%% For resonances like "N(1440)P_11" (all arguments ``spelled out'')
\DeclareRobustCommand{\HepParticleResonanceFormalFull}[9]{%
  \HepParticleResonanceFormal{\HepParticle{#1}{#2}{#3}}{#4}{#5}{#6}{#7}{#8}{#9}%
}


%% For typesetting HEP processes with these particle names.
%% TODO: Help on how to widen the math spacing would be nice: I always
%% find myself putting \, between particle names to make it look good.
\let\@HepOldto\to
\DeclareRobustCommand{\HepProcess}[1]{%
  \begingroup%
  \renewcommand{\to}{\mspace{1mu}\@HepOldto\mspace{1mu}}%
  \ensuremath{#1}%
  \renewcommand{\to}{\@HepOldto}%
  \endgroup%
}


%% Typesetting tweaks (-> becomes "to", remove mspace) from hyperref labels in PDFTeX
%% Thanks to Heiko Oberdiek and Donald Arseneau for assistance via comp.text.tex
\@ifpackageloaded{hyperref}{
  \pdfstringdefDisableCommands{%
      \DeclareRobustCommand{\HepProcess}[1]{#1}
      \let\mspace\@gobble
      \def\to{to }%
  }%
}{}

